Neural Unbalanced Optimal Transport via Cycle-Consistent Semi-Couplings

Comparing unpaired samples of a distribution or population taken at different points in time is a fundamental task in many application domains where measuring populations is destructive and cannot be done repeatedly on the same sample, such as in single-cell biology. Optimal transport (OT) can solve this challenge by learning an optimal coupling of samples across distributions from unpaired data. However, the usual formulation of OT assumes conservation of mass, which is violated in unbalanced scenarios in which the population size changes (e.g., cell proliferation or death) between measurements. In this work, we introduce NubOT, a neural unbalanced OT formulation that relies on the formalism of semi-couplings to account for creation and destruction of mass. To estimate such semi-couplings and generalize out-of-sample, we derive an efficient parameterization based on neural optimal transport maps and propose a novel algorithmic scheme through a cycle-consistent training procedure. We apply our method to the challenging task of forecasting heterogeneous responses of multiple cancer cell lines to various drugs, where we observe that by accurately modeling cell proliferation and death, our method yields notable improvements over previous neural optimal transport methods.

==> content/notes.tex <==

\section{David' note - remove eventually}

%($Tx_i$, $\mathbf{u}_i h_`(x_i)/$
 





%  for a pair of optimal forward/backward transport maps $T,S$. 


% How are $\tilde{\mu}$ and $\tilde{\nu}$ to be chosen? Given an \textit{ansatz} for the forward map $T: \gX \rightarrow \gX$, our 



%For a pair of candidate forward and backward maps $T,S: \gX \rightarrow \gX$, we want 


%  i.e., we seek   which satisfy 

By doing so, we can decompose the unbalanced problem as a sequence of measure scaling, mapping, measure scaling operations. 


\dam{Might want to discuss why not directly computing the UBOT between $\mu$ and $\nu$ to get the required weights. The issue with this is that we don't want to naively find \textit{any} reweighting that gives us the right maringals. Comparing $\mu$ and $\nu$ without first mapping them will likely lead to uniformative UBOT couplings. Also, they would be static throughout training. Instead, we want to refine our estimates of the mass correspondence (and therefore, reweigiting necessary) as we nail down the (feature to feature) correspondence between them}. 





\todo{

Issues, no Brenier (but a dual), no mapping, crucial for neural OT (out-of-sample)

We try to bind semi-coupling with previous parameterizations of the Monge maps

Intuition

(diagram)

Formalization and how to use Makkuva in the core
Objective

Optimality and cycle-consistency


Algorithm and training (e.g., use unbalanced OT from POT to achieve this) etc.

}







Notation: Let $\hat{\mu} = \nabla g_\sharp \mu , \tilde{\mu} = \eta \cdot \mu$, and $\hat{\tilde{\mu}} = \nabla (g_\sharp \mu) \cdot \eta = \nabla g_\sharp (\eta \cdot \mu)$. Here, $\eta \cdot \mu$ means that every $x$ has mass $\eta(x)\mu(x)$, though I'm not sure this is a valid formal definition. Analogously for the target distribution we have: $\hat{\nu} = \nabla f_\sharp \nu , \tilde{\nu} = \zeta \cdot \nu$, and $\hat{\tilde{\nu}} = \nabla (f_\sharp \nu) \cdot \zeta = \nabla f_\sharp (\zeta \cdot \nu)$. 

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/IMG_5961_small.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

In the Algorithm (L4) we compute $\hat{\mu} \eqdef  \nabla g_\sharp \mu$ and solve UBOT between it and $\nu$, obtaining $\Gamma_1$ (L6). Since this is an UBOT problem, $\Gamma_1$'s marginals are typically not equal to $(\hat{\mu},\nu)$. Its actual marginals can be written (using Chizat's notation for projection of a coupling) as $((\Proj_0)_\sharp \Gamma_1, (\Proj_1)_\sharp \Gamma_1)$. We define $\tilde{\mu}$ as the first of these, hence $\Gamma_1$ is a valid (balanced) coupling between $\tilde{\mu}$ and $(\Proj_1)_\sharp \Gamma_1$. In L7 we're defining $\eta$ to satisfy $\eta \cdot \mu = (\Proj_0)_\sharp \Gamma_1 = \tilde{\mu}$, that is, the reweighting needed to conform $\mu$ to $\Gamma_1$'s first marginal. Note that don't explicitly compute $\tilde{\mu}$, we just know it can be obtained from $\eta$ and $\mu$. Similarly, we implicitly define $\hat{\tilde{\mu}} = \nabla g_\sharp (\eta \cdot \mu)$.

Analogously,  we compute $\hat{\nu} \eqdef \nabla f_\sharp \nu $ (L5), and solve UBOT between it and $\mu$, obtaining $\Gamma_2$ (L8). $\Gamma_2$'s marginals are $((\Proj_0)_\sharp \Gamma_2, (\Proj_1)_\sharp \Gamma_2) \eqdef (\tilde{\nu}, (\Proj_1)_\sharp \Gamma_2)$. In L9 we're defining $\zeta$ to satisfy $\zeta \cdot \nu = (\Proj_0)_\sharp \Gamma_2 = \tilde{\nu}$. Finally, we implicitly define $\hat{\tilde{\nu}} = \nabla f_\sharp (\zeta \cdot \nu)$.

The objective in L10 corresponds to (Makkuva's formulation of) the 2-Wasserstein objective between $\tilde{\mu}$ and $\tilde{\nu}$, which can be seen by writing its population version as:

\begin{align*}
    \mathcal{L}(f,g) &= \int_\mathcal{X} \bigl[ f(\nabla g (x)) - \langle x, \nabla g (x) \rangle \bigr ] \eta(x) \dif \mu(x)- \int f(y) \zeta(y) \dif \nu(y) \\
    &= \Exp_{x\sim \tilde{\mu}} \left[ f (\nabla g) - \langle x, \nabla g (x) \rangle \right ] -  \Exp_{y\sim \tilde{\nu}} \left[ f(y) \right]
\end{align*}

Thus, at optimality $(f,g)$ are the katorovich potentials, so we have
\begin{align*}
    \hat{\tilde{\mu}} \eqdef \nabla g_\sharp \tilde{\mu}  \approx \tilde{\nu}  \qquad \text{and} \qquad  \hat{\tilde{\nu}} \eqdef \nabla f_\sharp \tilde{\nu}  \approx \tilde{\mu} 
\end{align*}


Other observations
\begin{itemize}
    \item This derivation provides a plausible explanation for Frederike's observation that $\tilde{\mu} = \eta \cdot \mu \approx \zeta \cdot \nu = \tilde{\nu}$ for every cluster. At optimality  we have $\tilde{\nu} \approx \nabla g_\sharp {\tilde{\mu}}$ (see diagram). Let $A$ be a set (e.g., cluster) for which $\nabla g$ preserves mass (formally, it is a measure-preserving map when restricted to $A$). Then 
    \[ \tilde{\nu}(A) = \int_{A} \dif \tilde{\nu} 
    \stackrel{\text{(optimality)}}{\approx}  \int_A \dif \nabla g_\sharp {\tilde{\mu}} \stackrel{\text{(def.~of }\sharp)}{=}  \int_A \nabla g  \dif\tilde{\mu} \stackrel{\text{(measure preserv.)}}{=} \int_A \dif \tilde{\nu} = \tilde{\mu}(A)\]
    Whenever our Monge maps are reasonable, they should be measure preserving within any cluster, so the above would hold (perhaps approximately) when looking at every cluster. 
    % \item Let  $\hat{\Gamma_1}$ be the trivial coupling constructed from $P_y\Gamma_1$, i.e.,  $\hat{\Gamma_1}(y,y') = \nu(y')$ if $y=y'$ and zero otherwise (in the discrete case, it would be a diagonal matrix $\text{diag}(\mathbf{b}))$. Claim: ($\Gamma_1$, $\hat{\Gamma_1}$ ) is a valid semi-coupling pair between $\mu$ and $\nu$. Proof: $\Gamma_1$ has left-marginal $\tilde{mu}$ by definition. Since $\nabla g$ is a deterministic map, then $\Gamma_1$ implicitly provides a 
    \item From the above, we can define a valid pair of semi couplings between $\mu$ and $\nu$ as follows. Let $\Gamma^*_a$ be the trivial coupling between $\mu$ and $\tilde{\mu}$, i.e.,  $\Gamma^*_a(x,x') = \mu(x')$ if $x=x'$ and zero otherwise (in the discrete case, it would be a diagonal matrix $\text{diag}(\mathbf{a}))$. The chain together (need to formalize) $\nabla g$ and  $1/\zeta$ to get $\Gamma^*_b$ with right-marginal $\nu$. Note that this pair satisfies $(\text{Proj}_1)_\sharp \Gamma^*_a = (\text{Proj}_0)_\sharp \Gamma^*_b$, which is not necessary. We can aslo define a non-matching pair of couplings as follows. Take $\Gamma^*_a$ as the chaining (formalize) of $\eta$ and $\Gamma_1$, so that it has marginals $\mu$ and $(\text{Proj}_1)_\sharp \Gamma_1$. Analogously define $\Gamma^*_b$ by chaining $\Gamma_2^\top$ and $\zeta$ so that it has marginals  $(\text{Proj}_0)_\sharp \Gamma_2$ and $\nu$. Boom! Done!
\end{itemize}



\dam{Not sure if we need this but typing it up for the purposes of discussion}

\begin{equation}
    \sup_f \inf_g \mathcal{V}_{\mu,\nu}(f,g) + C_{\mu,\nu} = \sup_f \inf_g -\Exp_{\mu}[f(X)] - \Exp_{\nu}\bigl[ \langle Y, \nabla g(Y) \rangle - f(\nabla g(Y)) \bigr] + C_{\mu, \nu} = 
\end{equation}

\begin{equation*}
    J(\theta_g, \theta_f) = \mathbb{E}_{x\sim \tilde{\mu}} \bigl[ f(\nabla g(x)) - \langle x, \nabla g(x)) \bigr]  - \mathbb{E}_{y \sim \tilde{\nu}} f(y) 
\end{equation*}
                 
...

